Arbitrarily Varying Remote Sources

We study a lossy source coding problem for an arbitrarily varying remote source (AVRS) which was proposed in a prior work. An AVRS transmits symbols, each generated in an independent and identically distributed manner, which are sought to be estimated at the decoder. These symbols are remotely generated, and the encoder and decoder observe noise corrupted versions received through a two-output noisy channel. This channel is an arbitrarily varying channel controlled by a jamming adversary. We assume that the adversary knows the coding scheme as well as the source data non-causally, and hence, can employ malicious jamming strategies correlated to them. Our interest lies in studying the rate distortion function for codes with a stochastic encoder, i.e, when the encoder can privately randomize while the decoder is deterministic. We provide upper and lower bounds on this rate distortion function.

==> bkdproof.tex <==
\ajb{The set of all claims/lemmas with proofs.}
\begin{claim}
There exists a $\dtwod,\fone>0$, where $\dtwod,\fone\rightarrow 0$
as $\delta,\epsilon\rightarrow 0$,
%and $n$ large enough 
such that the encoder
finds a codeword $\bU$ with probability at least $1-2^{-n\fone}$ such that
$(\bY,\bU)\in\cT^n_{\dtwo}(P_{U|Y}T_{\bY})$. 
% this probability is at least $(1-\epsilon')$, where $\epsilon'$ is double exponentially vanishing. 2^{-2^{n\delta/4}}
\end{claim}
The proof of this claim follows from the covering lemma~\cite[Lemma~3.3]{elgamal-kim}. As our choice of $R_U(T_{\bY})=I_{P_{U|Y}T_{\bY}}(U;Y)+\epsilon/4$, we choose a $\dtwod$ small enough. Note that this  specifies the $\dtwod$ parameter which appears in the definition of the encoder in~\eqref{eq:encoder:condition:dmc}.
We define this ``good'' encoder event as $E_{enc}:=\{(\bY,\bU)\in\cT^n_{\dtwo}(P_{U|Y}T_{\bY})\}$.
%
\begin{claim}
Let $\dnot=\delta/2$, and
let $\bX$ be generated i.i.d. $\sim P_X$. Then, with probability at least $(1 - |\cX|e^{-2n\dnot^2})$, $\bX \in 
\cT^n_{\dnot}(P_X)$.
\end{claim}
Let us define this ``good'' event as $E_{x}:=\{\bX \in \cT^n_{\dnot}(P_X)\}$.
%
\begin{claim}\label{lem:j:typ:x}
Let $(\vec{x},\vec{j})$ be a pair of vectors where $\vec{x}\in\mathcal{T}_{\dnot}^n(P_X)$.
Then, $(\vec{x},\vec{j})\in \mathcal{T}_{\dnot}^n(P_{X} T_{\vec{j}|\vec{x}})$.
\end{claim}
%
Let us denote the event that $(\bX,\bJ)$ is jointly typical w.r.t. $P_X T_{\bJ|\bX}$ as $E_{x,j}$. By the above claim, we have $E_{x} \subseteq E_{x,j}$.
%
\begin{lemma}[Conditional typicality lemma]\label{lem:cond:typ}
Let $\bs\in\cT^n_{\dnot}(P_S)$ and $\bT$ be generated from $\bs$ using the memoryless distribution $W_{T|S}$. Then,
%
\begin{IEEEeqnarray}{rCl}
\mathbb{P}\left((\bs,\bT)\in\cT^n_{3\dnot}(P_S W_{T|X})\right)\geq 1-|\cS||\cT| e^{-2 n\delta^3_0}.\label{eq:P:s:t}
\end{IEEEeqnarray}
%
\end{lemma}
%
\begin{IEEEproof}
We need to show that
%
\begin{align*}
&\mathbb{P} \left(\left|T_{\bs,\bT}(s,t)-P_S(s) W_{T|S}(t|s) \right| > 2\dnot\right) 
\end{align*}
is exponentially small for all $s,t$.
We consider two cases. \\
{\it Case I:} $T_{\bs}(s)\leq \dnot$.
As $\bs\in\cT^n_{\dnot}(P_S)$, this implies that 
$ P_S(s)\leq T_{\bs}(s)+\dnot \leq 2\delta_0.  $
%
Then,~$\forall (s,t)$,
%
\begin{IEEEeqnarray*}{rCl}
\left|T_{\bs,\bT}(s,t)-P_S(s) W_{T|S}(t|s) \right| &=&\left|T_{\bs}(s)T_{\bT|\bs}(t|s)-P_S(s) W_{T|S}(t|s) \right|\\
&\leq& \max \left( T_{\bs}(s)T_{\bT|\bs}(t|s), P_S(s)W_{T|S}(t|s)\right)  \\
&\stackrel{}{\leq}& 2\dnot \cdot 1  \\
&=&2\dnot.
\end{IEEEeqnarray*}
%
Thus, for such $s$, $\bbP \left(\left|T_{\bs,\bT}(s,t)-P_S(s) W_{T|S}(t|s) \right| > 2\dnot\right)=0$.\\
{\it Case II:} $T_{\bs}(s)> \dnot$.
Using Chernoff-Hoeffding's  theorem~\cite[Theorem~1]{hoeffding-1963} for each $t\in\cT$, we have
%
\begin{IEEEeqnarray*}{rCl}
\mathbb{P}(|W_{T|S}(t|s)-T_{\bT|\bs}(t|s)| >\dnot, \text{ for any } t ) \leq |\cT|e^{-2n \delta^3_0 }.
\end{IEEEeqnarray*}
%
Now, it can be easily checked that 
$|W_{T|S}(t|s)-T_{\bT|\bs}(t|s)| \leq \dnot$ and $|P(s)-T_{\bs}(s)| \leq
\dnot$ together imply 
$$\left|T_{\bs}(s)T_{\bT|\bs}(t|s)-P_S(s) W_{T|S}(t|s) \right| \leq 2\dnot+\dnot^2 \leq 3\dnot.$$
%
Hence,~\eqref{eq:P:s:t} follows by taking union bound over all $s\in\cS$.
%
\end{IEEEproof}

\begin{claim}
With probability at least $(1-|\cX||\cJ||\cY||\cZ|e^{-2 \dnot^3 n})$,  $(\bX,\bJ,\bY,\bZ)$ are jointly $3\dnot$-typical according to the distribution $P_S T_{\bJ|\bX} W_{Y,Z|X,J}$.
\end{claim}
The proof of this result follows from Lemma~\ref{lem:cond:typ}.
We define this ``good'' event as $E_{x,j,y,z}:=\{(\bX,\bJ,\bY,\bZ)
\in \cT_{3\dnot}^n(P_X T_{\bJ|\bX} W_{Y,Z|X,J})\}$.
%
\begin{claim}
Under the event $E_{x,j,y,z}$, the vector $\bY$ is $\done$-typical w.r.t. $P_Y=[P_XT_{\bJ|\bX}W_{Y,Z|X,J}]_Y$, where $\doned=3|\cX||\cJ||\cZ|\dnotd\rightarrow 0$ as $\delta\rightarrow 0$. That is,
$\|T_{\bY} - P_Y\|_{\infty} \leq 3|\cX||\cJ||\cZ|\dnot$. 
\end{claim}
The proof is straightforward, and hence, omitted. The above claim implies that, except for an exponentially small probability,
the decoder considers the conditional type $T_{\bJ|\bX}$ for decoding.
%
\begin{claim}\label{claim:y:u:tpy}
Under $E_{enc}$ and $E_{x,j,y,z}$, $(\bY,\bU)$ are jointly $\dthree$-typical according to the distribution 
$P_Y P_{U|Y}$, where 
$P_Y=[P_XT_{\bJ|\bX}W_{Y,Z|X,J}]_Y$ and
$\dthreed:=3|\cX||\cY||\cZ|\dnotd + \dtwod \rightarrow 0$ as $\delta \rightarrow 0$.
\end{claim}
\begin{IEEEproof}
Note that
\begin{align*}
\|P_YP_{U|Y} - T_{\bU\bY}\|_{\infty} & \leq \|P_YP_{U|Y} - T_{\bY}P_{U|Y}\|_{\infty}
               + \|T_{\bY}P_{U|Y} - T_{\bU\bY}\|_{\infty}\\
& \leq 3|\cX||\cY||\cZ|\dnot + \dtwo \quad \text{(using $E_{enc}$ and $E_{xjyz}$)}\\
& = \dthree,
\end{align*}
where $\dthree=3|\cX||\cY||\cZ|\dnot + \dtwo$.
\end{IEEEproof}
%
\begin{claim}\label{claim:unif:dist}
%
There exists $g(\delta)>0$, where $g(\delta)\rightarrow 0$ as $\delta\rightarrow 0$, such that $\forall \bu\in\cT^n_{\dthree}(P_{U|Y}P_Y|\by)$,
%
\begin{IEEEeqnarray}{rCl}\label{eq:tdX:dist}
P_{\bU}(\bU =\bu|\bY=\by)\leq 2^{-n(H(U|Y) -g(\delta) )}.
\end{IEEEeqnarray}
where $H(U|Y)$ is computed with the distribution $P_{U|Y}P_Y$.
%
%
\end{claim}
%
\begin{IEEEproof}[Proof of claim]
We have two cases.\\
{\it Case 1:} When $\bu\in \cT^n_{\dtwo}(P_{U|Y}T_{\by}|\by) \bigcap \cT^n_{\dthree}(P_{U|Y}P_Y|\by)$.
Then we note that 
%
\begin{IEEEeqnarray*}{rCl}
&\mathbb{P} &\left( \bU =\bu|\bY=\by \right) \\
&\stackrel{}{=}& \mathbb{P} \left( \bU=\bu,\bU \in\cT^n_{\dthree}(P_{U|Y}T_{\by}|\vec{y})\big|\bY=\by  \right)\\
&=&\mathbb{P} \left( \bU \in\cT^n_{\dthree}(P_{U|Y}T_{\by}|\vec{y})\big|\bY=\by\right)\mathbb{P} \left( \bU=\bu\big|\bY=\by, \bU \in\cT^n_{\dthree}(P_{U|Y}T_{\by}|\vec{y}) \right)\\
&\leq& \mathbb{P} \left( \bU=\bu\big|\bY=\by, \bU \in\cT^n_{\dthree}(P_{U|Y}T_{\by}|\vec{y}) \right)\\
&=& \mathbb{P} \left( \bU_{1,1}=\bu\big|\bY=\by, \bU_{1,1} \in\cT^n_{\dthree}(P_{U|Y}T_{\by}|\vec{y}) \right)\footnote{
For our own record, the justification for this step is:
\begin{align*}
& \mathbb{P} \left( \bU=\bu\big|\bY=\by, \bU \in\cT^n_{\dthree}(P_{U|Y}T_{\by}|\vec{y}) \right)\\
= & \sum_{l\geq 1} P\left(|\cL|= l|\bY=\by, \bU \in\cT^n_{\dthree}(P_{U|Y}T_{\by}|\vec{y})\right) \sum_{i=1}^l \frac{1}{l} P\left(L_i = \bu|\bY=\by, \bU \in\cT^n_{\dthree}(P_{U|Y}T_{\by}|\vec{y}), |\cL|= l\right)\\
= & \sum_{l\geq 1} P\left(|\cL|= l|\bY=\by, \bU \in\cT^n_{\dthree}(P_{U|Y}T_{\by}|\vec{y})\right) \sum_{i=1}^l \frac{1}{l} \mathbb{P} \left( \bU_{1,1}=\bu\big|\bY=\by, \bU_{1,1} \in\cT^n_{\dthree}(P_{U|Y}T_{\by}|\vec{y}) \right)\\
= & \mathbb{P} \left( \bU_{1,1}=\bu\big|\bY=\by, \bU_{1,1} \in\cT^n_{\dthree}(P_{U|Y}T_{\by}|\vec{y}) \right)
\end{align*}
}\\
&=& \frac{\mathbb{P} \left( \bU_{1,1}=\bu|\bY=\by\right)}{ \mathbb{P}\left(\bU_{1,1} \in\cT^n_{\dthree}(P_{U|Y}T_{\by}|\vec{y})|\bY=\by \right)}\\
&\stackrel{}{\leq}& 2\cdot \mathbb{P} \left( \bU_{1,1}=\bu|\bY=\by\right)
\quad \text{(since  $\mathbb{P}\left(\bU_{1,1} \in\cT^n_{\dthree}(P_{U|Y}T_{\by}|\vec{y})|\bY=\by \right) \rightarrow 1$ as $n\rightarrow \infty$)}\\
&\stackrel{}{\leq}& 2^{-n(H_{P_{U|Y}T_{\by}}(U|Y) -g_1(\dthree) )}
%&\stackrel{(c)}{\leq}& \sum_{M=m} \mathbb{P} \left( M=m\big|\bY=\by, \bU_M \in\cT^n_{\delta}(P_{Y,Z}|\vec{y}) \right) 2^{-n(H(Z|Y) -g(\delta) )}\\
\end{IEEEeqnarray*}
where $g_1(\dthree)\rightarrow 0$ as $\dthree\rightarrow 0$.
Since $||P_Y - T_{\by}||_1 \leq |\cY|\cdot ||P_Y - T_{\by}||_\infty
\leq 3|\cX||\cJ||\cZ||\cY|\dnot$, and
$||P_YP_{U|Y} - T_{\by}P_{U|Y}||_1 \leq |\cU||\cY|\dthree$,
using \cite[Lemma~2.7]{csiszar-korner-book2011}, we get
%
\begin{IEEEeqnarray*}{rCl}
& |H_{P_Y}(Y) - H_{T_{\by}}(Y)| \leq 3|\cX||\cJ||\cZ||\cY|\dnot\cdot\log\left(
\frac{1}{3|\cX||\cJ||\cZ|\dnot}\right)\\  
& |H_{P_YP_{U|Y}}(U,Y) - H_{T_{\by}P_{U|Y}}(U,Y)| \leq |\cU||\cY|\dthree\cdot
\log\left( \frac{1}{\dthree}\right)  
\end{IEEEeqnarray*}
%
Together, the above two equations imply
\begin{align}
& |H_{P_YP_{U|Y}}(U|Y) - H_{T_{\by}P_{U|Y}}(U|Y)| \leq 2|\cU||\cY|\dthree\cdot
\log\left( \frac{1}{\dthree}\right). \label{eq:H:u:y}
\end{align}
By defining $g_2(\dthree) := g_1(\dthree) + 2|\cU||\cY|\dthree\cdot
\log\left( \frac{1}{\dthree}\right)$, we get
\begin{align*}
\mathbb{P} \left( \bU =\bu|\bY=\by \right)
& \stackrel{}{\leq} \frac{1}{2}\cdot 2^{-n(H_{P_{U|Y}P_{Y}}(U|Y) -g_2(\dthree) )}.
\end{align*}
{\it Case II:} 
When $\bu\not\in \cT^n_{\dtwo}(P_{U|Y}T_{\by}|\by) $. For such a $\bu$,
the encoder outputs it only if $\bU_{1,1}= \bu$ and there is no codeword
which is jointly typical with $\by$ w.r.t. $P_{U|Y}T_{\by}$.
Thus,
\begin{align*}
\bbP\left( \bU =\bu|\bY=\by \right)
& \stackrel{}{\leq} \bbP\left( \bU_{1,1} =\bu|\bY=\by \right)\\
& \leq 2^{-n(H_{[P_{U|Y}T_{\by}]_U}(U) - g_3(\dtwo))}\\
& \leq 2^{-n(H_{[P_{U|Y}P_Y]_U}(U) - g_4(\dtwo))},
\end{align*}
where $g_4(\dtwo) = g_3(\dtwo) + |\cU|^2|\cY|\dthree\cdot \log\left(
\frac{1}{|\cU||\cY|\dthree}\right)$.

Combining the two cases, and taking $g(\delta) = \max (g_2(\dthree),
g_4(\dthree))$, the lemma follows.
\end{IEEEproof}
%
\begin{lemma}[Refined Markov Lemma~\cite{bdp-arxiv2016}~\footnote{In the refined
Markov lemma presented in~\cite{bdp-arxiv2016}, condition (b) also has a lower
bound on $P_{\bZ}(\bz)$. However, the lower bound is not used in the proof
given in \cite{bdp-arxiv2016},
and hence, can be removed. Here, we state this lemma without any lower
bound. 
We also note that condition (a) and the upper
bound on the probability of a typical sequence imply that probability
of too many typical sequences can not be too small; and so some essence
of the lower bound in condition (b) is already implied by these. 
So it is not surprising that the lower bound is not needed for the 
lemma to hold.
}]\label{lem:ref:markov:lemma}
Suppose $X\rightarrow Y\rightarrow Z$ is a Markov chain, i.e., $P_{X,Y,Z}=P_{Y}P_{X|Y} P_{Z|Y} $. Let $(\vec{x},\vec{y})\in \mathcal{T}^n_{\dnot}\left(P_{X,Y}\right)$ and $\vec{Z} \sim P_{\vec{Z}}$ be such that
%
\begin{enumerate}[(a)]
\item $\mathbb{P}\left((\vec{y},\vec{Z})\not\in
\mathcal{T}^n_{\dnot}\left(P_{Y,Z}\right)\right)\leq \epsilon$, where $\epsilon>0$,
%$\epsilon_n\rightarrow 0$ as $n\rightarrow \infty$.
%, where $P_{Y,Z}^{(n)}=P_{Y}^{(n)}P_{Z|Y}$, and

\item for every $\vec{z}\in \mathcal{T}^n_{\dnot}\left(P_{Y,Z}|\vec{y}\right)$,
%
\begin{equation*}\label{eq:condition:markov}
P_{\vec{Z}}(\vec{z})\leq 2^{-n(H(Z|Y)-g(\dnot))},
\end{equation*}
for some $g:\mathbb{R}^{+}\rightarrow\mathbb{R}^{+}$, where $g(\dnot)\rightarrow 0$ as $\delta_0\rightarrow 0$.
%
\end{enumerate}
Then, there exists $\delta:\mathbb{R}^{+}\rightarrow\mathbb{R}^{+}$, where $\delta (\dnot) 
\rightarrow 0$ as $\dnot \rightarrow 0$, such that
%
\begin{equation*}
\mathbb{P}\left((\vec{x},\vec{y},\vec{Z})\not \in \mathcal{T}^n_{\delta(\dnot)}\left(P_{X,Y,Z}\right)   \right)\leq 2|\cX||\cY||\cZ| e^{-n K} +\epsilon.
\end{equation*}
%
Here $K>0$ and $K$ does not depend on $n$, $P_{X,Y}$, $P_{\vec{Z}}$ or $(\vec{x},\vec{y})$ but does depend on $\dnot$, $g$ and $P_{Z|Y}$. Further, the $\delta$ function does not depend on $(\bx,\by)$, $P_{X,Y}$ or $P_{\bZ}$.
%\ajblue{AJB: All references to dependence on $P_{Z|Y}$ and not on $P^{\min}_{Z|Y}$. }
%$P^{\min}_{Z|Y}:=\min_{(y,z) : P_{Z|Y}(z|y)>0} P_{Z|Y}(z|y)$.  
\end{lemma}
%
We now use the above lemma to prove the following claim.
%
\begin{claim}\label{claim:x:2:u:typ}
 There exists $\dfourd>0$, where $\dfourd\rightarrow 0$ as
$\delta\rightarrow 0$, such that except for an exponentially small
probability, $(\bX,\bJ,\bZ,\bY,\bU)$
is jointly $\dfour$-typical w.r.t. $P_XT_{\bJ|\bX}W_{YZ|XJ}P_{U|Y}$.
\end{claim}
\begin{IEEEproof}
Let us assume that $E_{x,j,y,z}$ is true.
Now we use the refined Markov lemma (Lemma~\ref{lem:ref:markov:lemma}) on the Markov chain $(X,J,Z) \rightarrow
Y \rightarrow U$.
Then, by Claims~\ref{claim:y:u:tpy} and~\ref{claim:unif:dist}, $\bU$ is chosen such that both
conditions (a) and (b) in Lemma~\ref{lem:ref:markov:lemma} are satisfied.
Thus, the claim follows.
\end{IEEEproof}
%
We define this ``good'' event as $E_{x,j,y,z,u}:=\{(\bX,\bJ,\bZ,\bY,\bU)
\in \cT^n_{\dfour}(P_XT_{\bJ|\bX}W_{YZ|XJ}P_{U|Y}\}$.
%
\begin{claim}
There exists $\gamma(\delta)>0$, where $\gamma(\delta)\rightarrow 0$ as $\delta\rightarrow 0$, such that except for an exponentially small probability, $\bU\in \cL_{\gamma(\delta)}(M,\bZ)$. 
\end{claim}
%
\begin{IEEEproof}
Consider the event $E_{x,j,y,z,u}$. Under this event, $(\bU,\bZ)$ are
$\gammad$-typical w.r.t. $P_{U,Z}=[P_X T_{\bJ|\bX} W_{Y,Z|X,J}
P_{U|Y}]_{U,Z}$, where $\gammad=|\cX||\cJ| |\cY| \dfour $. 
Thus, the claim follows from Claim~\ref{claim:x:2:u:typ}.
\end{IEEEproof}
%
This claim also specifies the $\gamma(\delta)$ parameter which appears in the definition of the decoder in~\eqref{eq:dec:cond}.

\begin{claim}
There exists $f_2(\delta,\epsilon)>0$, where $f_2(\delta,\epsilon)\rightarrow 0$ as $\delta,\epsilon\rightarrow 0$, such that
%
\begin{IEEEeqnarray}{rCl}
\mathbb{P}\left(\vec{U}_{M,L'}\in \mathcal{L}_{\gamma(\delta)}(M,\vec{Z}), \text{ for some } L'\neq L \right)\leq 2^{-n f_2(\delta,\epsilon)}.
\end{IEEEeqnarray}
%
\end{claim}
%
\begin{IEEEproof}
Note that the codewords $\{\bU_{M,L'}\}_{L'\neq L}$ and $\bZ$ are independent by construction. Let us consider a fixed conditional type $T_{J|X}\in \sQ(T_{\bY})$. Let the resulting joint distribution $P_{U,Z}=[P_X T_{J|X} W_{Y,Z|X,J} P_{U|Y}]_{U,Z}$. Then,
%
\begin{align*}
\mathbb{P}\big(\exists L'\neq L:(\vec{U}_{M,L'},\bZ)\in \cT^n_{\gamma(\delta)} (P_{U,Z})) \leq  2^{-n\tdftwo}
\end{align*}
for some $\td{\ftwo} \rightarrow 0$ as $\delta, \epsilon \rightarrow 0$. This follows from the packing lemma~\cite[Lemma~3.1]{elgamal-kim}. 
By taking the union bound over all conditional types $T_{J|X}\in\sQ(T_{\bY})$ (the number of such types is at most polynomial in $n$), we get
%
\begin{IEEEeqnarray*}{rCl}
\mathbb{P}\big(\exists L'\neq L: (\vec{U}_{M,L'},\bZ)\in \cT^n_{\gamma(\delta)} (P_{U,Z}) \text{  for some } T_{J|X}\in \sQ(T_{\bY})) &\leq& (n+1)^{|\cU||\cZ|} 2^{-n\tdftwo}\\
&\leq & 2^{-n\ftwo}.
\end{IEEEeqnarray*}
\end{IEEEproof}
%
%
\begin{claim}\label{claim:tdx}
There exists $r(\delta), f_3(\delta,\epsilon)$, where $r(\delta), f_3(\delta,\epsilon)\rightarrow$ as $\delta,\epsilon\rightarrow 0$, such that $\bbP\left(\bX,\btdX)\in \cT^n_{r(\delta)}(P_{X,\wtd{X}}\right)\geq 1-2^{-nf_3(\delta,\epsilon)}$.
\end{claim}
%
\begin{IEEEproof}
Recall Claim~\ref{claim:x:2:u:typ} which guarantees that $(\bX,\bJ,\bY,\bZ,\bU)$ are $\delta_4$-typical. Also, we know that $\vec{\wtd{X}}$ is a deterministic function $\vec{1}_{\{\wtd{X}=\td{x}(u,z)\}}$ of $(\bU,\bZ)$. Now using Lemma~\ref{lem:cond:typ}, we can directly conclude that with probability at least $(1-|\cX||\cJ||\cY||\cZ| |\cU||\ctdX|2^{-n\delta_4^3})$, we have $(\bX,\bJ,\bY,\bZ,\bU,\btdX)$ $3\delta_4$-typical, which further implies that $(\bX,\btdX)$ are $r(\delta)$-typical. Here $r(\delta):=3|\cX| |\ctdX| \delta_4(\delta)$. This completes the proof of the claim.
\end{IEEEproof}
%

